Composing Ensembles of Pre-trained Models via Iterative Consensus

Large pre-trained models exhibit distinct and complementary capabilities dependent on the data they are trained on. Language models such as GPT-3 are capable of textual reasoning but cannot understand visual information, while vision models such as DALL-E can generate photorealistic photos but fail to understand complex language descriptions. In this work, we propose a unified framework for composing ensembles of different pre-trained models -- combining the strengths of each individual model to solve various multimodal problems in a zero-shot manner. We use pre-trained models as "generators" or "scorers" and compose them via closed-loop iterative consensus optimization. The generator constructs proposals and the scorers iteratively provide feedback to refine the generated result. Such closed-loop communication enables models to correct errors caused by other models, significantly boosting performance on downstream tasks, e.g. improving accuracy on grade school math problems by 7.5%, without requiring any model finetuning. We demonstrate that consensus achieved by an ensemble of scorers outperforms the feedback of a single scorer, by leveraging the strengths of each expert model. Results show that the proposed method can be used as a general purpose framework for a wide range of zero-shot multimodal tasks, such as image generation, video question answering, mathematical reasoning, and robotic manipulation. Project page: https://energy-based-model.github.io/composing-pretrained-models.

==> text/method_backup.tex <==
subsection{Applications to Zero-shot Tasks}
\vspace{-3pt}
\textbf{Image generation.}
We first apply the proposed framework to image generation to generate images conditioned on a text description or a class label. 
% There is one image generator and multiple scorers that can provide feedback for the generated image. 
We use GLIDE~\citep{nichol2021glide}, a text-guided diffusion model, as the generator to generate image proposals. 
We then compose the generator with an ensemble of scorers, such as CLIP~\citep{radford2021learning}, to iteratively update the generated proposals based on the closed-loop communications between the models.
% , text-image classifiers~\citep{dhariwal2021diffusion}, and the classifier-free guidance~\citep{ho2022classifier}.

% , to provide feedback for the generator to refine the generated result. 

As shown in \cref{fig:model_details1} (b), the image $x_{t}$ generated at iteration $t$ is first sent to the GLIDE diffusion model to generate an image proposal $\hat{x}_{t+1}$. 
Each scorer outputs a score to evaluate whether the generated image matches the given text input. For example, CLIP computes the cosine distance between the image and text features. The image classifier predicts the probability of the image matching the text label. The classifier-free guidance can be treated as an implicit classifier that directly provides pixel-wise gradient feedback to the generated image.
The scores generated by different scorers are summed up, and their gradient with respect to $x_{t}$ is used to obtain $x_{t+1}$:
\vspace{-3pt}
\begin{equation}
    % x_{t+1}=x_t-\frac{\lambda}{2} \nabla_{x} \sum_{n=1}^N E_{\theta}^n \left(x_{t}, c \right),
    x_{t+1} =\mathcal{N}(\hat{x}_{t+1} + \lambda \nabla_{x} \sum_{n=1}^N E_{\theta}^n \left(x_{t}, c \right), \sigma^2),
\end{equation}
where $\mathcal{N}$ is the normal distribution, $N$ is the number of scorers and $\sigma^2$ is the variance. 



\textbf{Video question answering (VQA).}
We first use the proposed framework to generate video frame captions. We then use GPT-3 to summarize the captions and answer questions. 
As shown in \cref{fig:model_details1} (c), our framework combines GPT-2 and multiple CLIP models, trained with different configurations, for zero-shot video frame captioning.
Given a video frame and a text prompt, such as ``Image of'', we generate a sequence of words to describe the frame. Similar to \citep{tewel2021zero}, we define a context cache $C_t$ (a set of embedding functions in Transformer~\citep{vaswani2017attention}) that store the context information generated so far. The prediction of the next word can be written as $x_{t+1}=LM(x_t, C_t)$, where $LM$ is the language model (GPT-2). 
The goal is to update $C_t$ iteratively based on the CLIP score to generate the next word such that the sentence is grammatically sound as well as accurately describes the given video frame. 
To do this, we first use GPT-2 to generate a set of candidate words $\{\hat{x}_{t+1}^i\}$, and then use the feature distance between each sentence (the concatenation of previous words and each new word $\{x_1, x_2, \cdots, \hat{x}_{t+1}^i\}$) and the video frame as the probability of them matching. The CLIP score is the cross-entropy loss between this clip distribution and the original distribution of the next word obtained from GPT-2.
% The history tokens $\{x_1, \cdots, x_t\}$ is first sent to the generator to predict the next token $\hat{x}_{t+1}$.
% Then the scorers compute the feature distances (scores) between the new sentence (concatenation of history tokens and the new token) and the given video frame.
Similar to image generation, the gradient of summed scores (multiple CLIP models) is propagated to GPT-2 to update $C_t$. After several iterations, the updated $C_t$ is used to generate the next token $x_{t+1}=LM(x_t, C_t)$. We repeat this process until we generate the entire frame caption.
We cascade the video frame captions and questions about this video to prompt GPT-3 for video question answering.
% Results show that utilizing the proposed framework and GPT-3 enables effective video question answering.

% \begin{equation}
%     \sum_{n=1}^N E_{\theta}^n \left(x_1, \cdots, \hat{x}_{t+1}, c \right),
% \end{equation}



\textbf{Grade school math.}
We treat the grade school math problem as the text generation problem.
The generator is GPT-2. The scorer, a pre-trained question-solution classifier, provides the generator feedback to guide the next token's generation $x_{t+1}$. 
Similar to VQA, GPT-2 first generates a set of candidate words $\{\hat{x}_{t+1}^i\}$, and then the classifier predicts the probability of each solution (the concatenation of previous words and each new word $\{x_1, x_2, \cdots, \hat{x}_{t+1}^i\}$) matching the given question. 
The classifier score is the cross-entropy loss between this classifier distribution and the original distribution of the next word obtained from GPT-2. The gradient of the classifier score is used to update $C_t$ through iterative optimization. The updated $C_t$ is used to predict the next word $x_{t+1}=LM(x_t, C_t)$. We repeat this process until we generate the complete solution.





% The pre-trained scorer is a classifier to evaluate the correctness of the output answer for the given math problem.



% \input{compose-foundation-models/figs/model_details2}



\textbf{Robot manipulation.} Finally, we illustrate how \modelname can be applied to manipulate objects in the robot environment to conform to a set of object relations. 
The object relations are specified by text descriptions, such as ``orange mug to the right of orange bowl'', or real-world images that illustrate the relations. 
We use the combination of the Model Predictive Control (MPC) and the World Model as the generator.
At each time step, we first use MPC to sample a set of possible actions and then render the state images (after executing an action) from multiple camera views using the world model. For each action, the scorer computes a summed score across all camera views as its final score, which is used to select the best action to execute.

For the generator, we assume that there is a pre-trained model, \ie world model, that can accurately render and simulate the dynamic changes in the robot world. Since such a large pre-trained model does not directly exist, we approximate it using an environment simulator combined with MPC as the generator.
For the scorer, we use ViLD~\citep{gu2021open} to generate segmentation maps for images captured by different camera views, and the corresponding text label for each segment, which are used to obtain object relations in the 3D world.
We compare the generated object relations and the relations specified by the text description or real-world image to obtain the scorer, \ie score equals 1 if they match; otherwise, 0.
We combine the scores from multiples camera views and used \eqn{eq:compose_energy} to select the best action at each time step.

% Given a pretrained ``world model'' of the world, we construct a set of different energy scorers, each of which takes a different rendered view of the world, and scores the extent to which the view satisfies a specified set of relations. We wish sample a set of object states of the world which maximize the score of energy scores (maximizing \eqn{eq:compose_energy}). To obtain such a set of objects, we utilize a MPC procedure, where we sample many different possible actions in the environment and choose the one  that leads to a world state with maximal score given by the energy scores.

% To construct our energy scorer, we use a pre-trained VLM VILD \citep{gu2021open} and crafted classifier. We run VILD on an input image, and obtain a segmentation of the world, and corresponding text-label for each segment. Given labeled segmentations, we manually construct a classifier which computes scores per object relation (details in Appendix). To construct different energy scorers, we render object states at a variety of different views.

% assess the extent to which relations are satisfied by the image, by back-projecting 2D segmentations to 3D pointclouds, and comparing the relative 3D offsets between segmented pointclouds. 




